DALK: Dynamic Co-Augmentation of LLMs and KG to answer Alzheimer's Disease Questions with Scientific Literature

Recent advancements in large language models (LLMs) have achieved promising performances across various applications. Nonetheless, the ongoing challenge of integrating long-tail knowledge continues to impede the seamless adoption of LLMs in specialized domains. In this work, we introduce DALK, a.k.a. Dynamic Co-Augmentation of LLMs and KG, to address this limitation and demonstrate its ability on studying Alzheimer's Disease (AD), a specialized sub-field in biomedicine and a global health priority. With a synergized framework of LLM and KG mutually enhancing each other, we first leverage LLM to construct an evolving AD-specific knowledge graph (KG) sourced from AD-related scientific literature, and then we utilize a coarse-to-fine sampling method with a novel self-aware knowledge retrieval approach to select appropriate knowledge from the KG to augment LLM inference capabilities. The experimental results, conducted on our constructed AD question answering (ADQA) benchmark, underscore the efficacy of DALK. Additionally, we perform a series of detailed analyses that can offer valuable insights and guidelines for the emerging topic of mutually enhancing KG and LLM. We will release the code and data at https://github.com/David-Li0406/DALK.

==> latex/1-introduction.tex <==
% introduction about LLMs
% LLMs limitation in long-tail/ domain-specific knowledge
% Large language models~(LLMs)~\citep{brown2020language,zhang2022opt,anil2023palm,touvron2023llama} have demonstrated strong capabilities across various tasks and applications~\citep{liang2022holistic,chang2023survey}.
% Recently, many chain-of-thought (CoT)-based methods~\cite{wei2022chain,wang2022self,li2023dail,tong2023eliminating,yao2023tree,besta2023graph} have been proposed to further unleash the \emph{reasoning} abilities of LLMs.
Large language models~(LLMs)~\citep{brown2020language,zhang2022opt,anil2023palm,touvron2023llama} with chain-of-thought (CoT)-based prompting~\cite{wei2022chain,wang2022self,li2023dail,tong2023eliminating,yao2023tree,besta2023graph} have demonstrated strong capabilities across various tasks and applications.
While they show promising performance in many general tasks, some recent studies expose LLMs' limitations in long-tail~\cite{kandpal2023large} and domain-specific~\cite{li2023multi,li2024contextualization} knowledge, thereby significantly impeding their adaptation in vertical fields such as biomedicine and finance~\cite{thirunavukarasu2023large,thapa2023chatgpt,yang2023fingpt,wu2023bloomberggpt}.

% previous solutions & their limitation
Previous works have proposed various approaches to address this challenge.
Existing methods can be roughly classified into three types: domain-specific LLMs training, document retrieval augmented generation (RAG), and knowledge graph-augmented LLMs.
% Domain-specific LLMs training~\cite{zhang2023biomedgpt,labrak2024biomistral,yang2023fingpt,wu2023bloomberggpt} requires collecting training data in a certain area to finetune or retrain a domain-specific LLM.
Training domain-specific Large Language Models (LLMs) ~\cite{zhang2023biomedgpt,labrak2024biomistral,yang2023fingpt,wu2023bloomberggpt} necessitates the accumulation of training data within a specific domain to fine-tune or retrain the LLM accordingly.
By contrast, RAG~\cite{gao2023retrieval,jeong2024improving,chen2024benchmarking} is designed to retrieve pertinent context as a supportive document during the inference phase.
Besides, there are also many works~\cite{wen2023mindmap,jiang2023structgpt} that concentrate on selecting relevant knowledge from knowledge graphs and integrating them into LLMs to enhance performance.

However, the abovementioned approaches still suffer from several limitations.
First, \textbf{Efficiency \& Scale Issues}: Retraining or fine-tuning a LLM demands substantial computational resources~\cite{hu2021lora,ovadia2023fine} and can lead to problems such as catastrophic forgetting (CF)~\cite{luo2023empirical}. 
These issues also limit the model sizes and scales of domain-specific LLMs (e.g., most of them only have 7B and 13B versions).
Second, \textbf{Data Quality}: Although the tuning-free nature of RAG enhances its efficiency and broad applicability, many specialized domains may still lack access to high-quality retrieval corpora. Previous research has shown that noisy and irrelevant corpora can significantly impact the performance of LLMs~\cite{yu2023chain,chen2024benchmarking,wu2024easily}.
Third, \textbf{Data Availablity}: While knowledge graphs offer cleaner and more specific data compared to raw text, their construction often relies on manual labor. Consequently, they often fall short in terms of coverage within various domain-specific areas~\cite{zhong2023comprehensive,Romano2023TheAK}.

These challenges underscore the need for a more efficient, robust, and automatic framework to equip LLMs with domain-specific knowledge.
In this paper, we focus our contribution in the setting of Alzheimer’s Disease~\footnote{https://doi.org/10.1002/alz.13016} (AD)-related question answering.
AD is a neurodegenerative disorder characterized by progressive declines in cognitive and functional status over a span of decades. According to the World Health Organization as of 2024~\footnote{https://www.who.int/news-room/fact-sheets/detail/dementia}, AD is the single most common form of dementia affecting more than 30 million people worldwide at present and potentially over 100 million by 2050 as global populations age. However, current AD drug/therapy developments are facing critical challenges with very limited FDA-approved treatments available, due to the lack of knowledge and understanding of the underlying etiological mechanisms of the disease progression. Although scientific literature and dedicated biomedical databases could embed rich sources of AD knowledge, manual review of relevant information is impossible due to the volume. LLM-based methods can effectively fill the gap with their powerful NLP capabilities and serve as efficient automatic approaches.  

% Our solution

To tackle the limitations of LLMs in this AD-specific scenario, we propose a \underline{D}ynamic Co-\underline{A}ugmentation of \underline{L}LMs and \underline{K}G (DALK) framework that facilitates mutual benefits between LLMs and knowledge graphs.
Initially, our framework tackles the data availability challenge by extracting structural knowledge from unstructured scientific literature and constructing a domain-specific knowledge graph tailored to AD.
We employ two widely utilized knowledge graph construction methods, namely pair-wise construction and generative construction, to comprehensively assess their impact on knowledge graph quality.
Then, we utilize a coarse-to-fine sampling method with a novel self-aware knowledge retrieval approach to select appropriate knowledge from the knowledge graph and thus further address the data quality problem.
Notably, the tuning-free nature of our framework significantly enhances efficiency and facilitates its application in large-scale and API-based language models~\cite{anil2023palm}.
In the evaluation section, we derive an Alzheimer's Disease question answering (ADQA) benchmark from existing general medical QA datasets with millions of samples filtered by a manually written keyword list and self-sampling of LLMs.
Our extensive experiment on ADQA demonstrates the effectiveness of our framework in domain-specific applications compared with biomedical models and other RAG methods.
Further evaluation and analysis provide valuable insights into constructing high-quality knowledge graphs and sampling accurate knowledge from them.

% Contribution

In summary, our contribution can be summarized as follows:
\begin{itemize}
    \item We identify the constraints of the current methods for LLMs in domain-specific areas and introduce a dynamic co-augmentation framework of the LLM and knowledge graph to address these issues.
    \item We apply our method to the AD-specific domain and build a new ADQA benchmark to conduct extensive experiments to demonstrate the effectiveness of our proposed approach.
    \item We delve into a comprehensive analysis of our proposed method and provide valuable insights and guidance on how to construct a high-quality knowledge graph and sample accurate knowledge from it.
\end{itemize}

==> latex/2-related-work.tex <==
% \subsection{Large Language Models and Knowledge Graphs}
\paragraph{The Interplay between LLMs and KGs}
KGs~\cite{miller1995wordnet,speer2017conceptnet,vrandevcic2014wikidata} serve as structured representations of factual knowledge, typically expressed as (head, relation, tail) triples.
Their structured, factual, and interpretable nature renders them excellent complements to parametric language models~\cite{pan2024unifying}.
Recently, with the rise of large language models (LLMs), numerous studies have delved into exploring the synergy between LLMs and KGs for various purposes.
There are a lot of efforts in conducting knowledge graph construction~\cite{carta2023iterative,wadhwa2023revisiting,han2023pive,bi2024codekgc,datta2024construction}, completion~\cite{wei2023kicgpt,zhang2023making,li2024contextualization} with the aid of LLMs.
Conversely, other works aim to enhance LLMs by integrating knowledge sampled from KGs during both training~\cite{tang2023graphgpt,luo2024knowla,dernbach2024glam,rangel2024sparql} and inference~\cite{kim2023kg,wen2023mindmap,jiang2023structgpt,sun2023think} times.
Our work distinguishes itself by proposing a co-augmentation framework for LLMs and KGs, facilitating their mutual enhancement, and applying it to the domain of AD.

% \subsection{NLP for Alzheimer’s Disease}
\paragraph{LLMs and KGs for AD research}
LLMs and KGs have both been applied to Alzheimer's Disease research in previous studies. 
Pre-trained language models have been utilized to work on AD detection and many other related tasks based on speech recordings and transcripts~\cite{balagopalan2020to, agbavor2022predicting}, electronic health records (EHRs)~\cite{mao2023ad,li2023two, yan2024leveraging}, and tabular data~\cite{feng2023large}. KGs have been widely used in biomedical research, yet only a few are specifically for AD research~\cite{romano2023the, pu2023graph, hsieh2023synthesize, yi2022mining, Geesa2023in}. These AD-KGs were generally constructed from a variety of information derived from heterogeneous biomedical databases (e.g. for genes, drugs, pathways, etc.) or scientific literature related to AD. Despite the aforementioned efforts for LLMs and KGs in AD research, no prior study has explored using LLM to augment AD-KG, or vice versa, let alone the potential for mutual enhancement between the two as we propose here.
